Error-Tolerant E-Discovery Protocols

We consider the multi-party classification problem introduced by Dong, Hartline, and Vijayaraghavan (2022) in the context of electronic discovery (e-discovery). Based on a request for production from the requesting party, the responding party is required to provide documents that are responsive to the request except for those that are legally privileged. Our goal is to find a protocol that verifies that the responding party sends almost all responsive documents while minimizing the disclosure of non-responsive documents. We provide protocols in the challenging non-realizable setting, where the instance may not be perfectly separated by a linear classifier. We demonstrate empirically that our protocol successfully manages to find almost all relevant documents, while incurring only a small disclosure of non-responsive documents. We complement this with a theoretical analysis of our protocol in the single-dimensional setting, and other experiments on simulated data which suggest that the non-responsive disclosure incurred by our protocol may be unavoidable.

==> Paper/critical.tex <==
\section{Critical} % (fold)
\label{sec:critical}


==> figures/1d_example.tex <==
\begin{figure}[H]
    \centering
    \begin{tikzpicture}
        \draw[->] (-1,-0.5) -- (6,-0.5) node[right] {$x$};
        \fill (5,-0.5) circle [radius=3pt];
        \fill (4,-0.5) circle [radius=3pt];
        \draw[red] (3,-0.5) circle [radius=3pt];
        \fill (2,-0.5) circle [radius=3pt];
        \fill (1,-0.5) circle [radius=3pt];
        \fill (0,-0.5) circle [radius=3pt];
        \node at (5,0) {+};
        \node at (4,0) {+};
        \node at (3,0) {-};
        \node at (2,0) {-};
        \node at (1,0) {-};
        \node at (0,0) {-};
        \node[blue] at (5,-1) {+};
        \node[blue] at (4,-1) {+};
        \node[blue] at (3,-1) {-};
        \node[blue] at (2,-1) {-};
        \node[blue] at (1,-1) {-};
        \node[blue] at (0,-1) {-};
        \node at (2.5, -1.5) {(a)};
    \end{tikzpicture}
    \begin{tikzpicture}
        \draw[->] (-1,-0.5) -- (6,-0.5) node[right] {$x$};
        \fill (5,-0.5) circle [radius=3pt];
        \fill (4,-0.5) circle [radius=3pt];
        \draw[red] (3,-0.5) circle [radius=3pt];
        \fill (2,-0.5) circle [radius=3pt];
        \fill (1,-0.5) circle [radius=3pt];
        \fill (0,-0.5) circle [radius=3pt];
        \node at (5,0) {+};
        \node at (4,0) {+};
        \node at (3,0) {-};
        \node at (2,0) {+};
        \node at (1,0) {-};
        \node at (0,0) {+};
        \node[blue] at (5,-1) {+};
        \node[blue] at (4,-1) {+};
        \node[blue] at (3,-1) {-};
        \node[blue] at (2,-1) {-};
        \node[blue] at (1,-1) {-};
        \node[blue] at (0,-1) {-};
        \node at (2.5, -1.5) {(b)};
    \end{tikzpicture}
    \caption{One-dimensional examples for realizable case (a) and non-realizable case (b). The top black labels are true labels of data points. The bottom blue labels are labels reported by the defendant. The red empty circle is the critical point in the critical points protocol. }
    \label{fig:example}
\end{figure}

